How Does Data Freshness Affect Real-time Supervised Learning?

In this paper, we analyze the impact of data freshness on real-time supervised learning, where a neural network is trained to infer a time-varying target (e.g., the position of the vehicle in front) based on features (e.g., video frames) observed at a sensing node (e.g., camera or lidar). One might expect that the performance of real-time supervised learning degrades monotonically as the feature becomes stale. Using an information-theoretic analysis, we show that this is true if the feature and target data sequence can be closely approximated as a Markov chain; it is not true if the data sequence is far from Markovian. Hence, the prediction error of real-time supervised learning is a function of the Age of Information (AoI), where the function could be non-monotonic. Several experiments are conducted to illustrate the monotonic and non-monotonic behaviors of the prediction error. To minimize the inference error in real-time, we propose a new "selection-from-buffer" model for sending the features, which is more general than the "generate-at-will" model used in earlier studies. By using Gittins and Whittle indices, low-complexity scheduling strategies are developed to minimize the inference error, where a new connection between the Gittins index theory and Age of Information (AoI) minimization is discovered. These scheduling results hold (i) for minimizing general AoI functions (monotonic or non-monotonic) and (ii) for general feature transmission time distributions. Data-driven evaluations are presented to illustrate the benefits of the proposed scheduling algorithms.

==> Abstract.tex <==
%!TEX root = ./AoI_LearningV3.tex
\begin{abstract}
This work analyzes the impact of data freshness on real-time supervised learning, where a neural network is trained to predict a time-varying target based on an observed feature. It is generally believed that the prediction error grows as the feature becomes stale. Our study shows that this is true if the feature and target data sequence can be closely approximated as a Markov chain; and not true if the data sequence is far from a Markov model, e.g., due to long-range dependence and communication delay. We consider the design of a feature communication system, in which a transmitter (e.g., a sensor or camera) sends features to a receiver that contains a neural network. By using the Gittins index theory, we develop an optimal feature buffering and transmission strategy that minimizes the prediction error and has low complexity. This result holds (i) for both Markovian and non-Markovian data, (ii) for general transmission time distributions from the transmitter to the receiver, and (iii) for a broad class of supervised learning algorithms. Numerical and experimental results are provided to illustrate our findings.
\end{abstract}

==> InformationFreshness.tex <==
%!TEX root = ./AoI_LearningV3.tex
\section{Information-theoretic Metrics for Real-time Forecasting (1 Page)}\label{InformationMetric}
\begin{figure*}[h]
  \centering
\begin{subfigure}{0.3\textwidth}
\includegraphics[width=\textwidth]{./Figure_Temperature/Temperature_Prediction.eps}
  \subcaption{Temperature Prediction}
\end{subfigure}
% <— this is important. There should be no empty line here. 
\begin{subfigure}{0.3\textwidth}
\includegraphics[width=\textwidth]{./Figure_CSI/CSI_Prediction.eps}
  \subcaption{CSI Prediction}
\end{subfigure}
%
\begin{subfigure}{0.3\textwidth}
\includegraphics[width=\textwidth]{./Figure_Cartpole/Cartpole_Angle.eps}
  \subcaption{CartPole Angle Prediction}
\end{subfigure}
%
\caption{Training error vs.~deterministic training AoI $\theta$ in three experiments: (a) temperature prediction, (b) wireless channel state information (CSI) prediction, and (c) angle prediction in CartPole balancing \cite{brockman2016openai}, where a Q-learning agent is used to control the cart and balance the pole.~When the length $u$ of the observation sequence $X_{t-\theta}=(s_{t-\theta}, \ldots, s_{t-\theta-u+1})$ is small, the training error may be non-monotonic in the training AoI $\theta$. As $u$ increases, the training error tends closer to a non-decreasing function of the training AoI $\theta$.}
\label{fig:Training}
\end{figure*}
The first goal of this paper is to interpret the role of information freshness in supervised learning based real-time forecasting. To that end, we will develop a theoretical foundation to characterize how training error $\mathrm{err}_{\mathrm{training}}$ and inference error $\mathrm{err}_{\mathrm{inference}}$ vary with the training AoI $\Theta$ and the inference AoI $\Delta$, respectively. {\violet It is well-known that finding analytical expressions for $\mathrm{err}_{\mathrm{training}}$ and $\mathrm{err}_{\mathrm{inference}}$ is quite difficult because the decision function $\phi$ represented by a neural network is highly complicated \cite{knight2017dark, castelvecchi2016can}.} In Sections \ref{InformationMetric} and \ref{InformationAnalysis}, we will address this challenge by modifying the goal and analyzing a fundamental lower bound of $\mathrm{err}_{\mathrm{training}}$, which can be expressed as a generalized conditional entropy $H_L(Y_t | X_{t-\Theta}, \Theta)$ {\blue that is mathematically more convenient to analyze}. 

\subsection{Metrics for Training Error}\label{SecMinTrainingError}
We bound {\blue the training error $\mathrm{err}_{\mathrm{training}}$ from below by the {generalized conditional entropy} $H_L(Y_t| X_{t-\Theta},\Theta)$ of $Y_t$ given $(X_{t-\Theta}, \Theta)$ \cite{Dawid2004, Dawid1998,farnia2016minimax}:}
\begin{align}\label{eq_TrainingErrorLB}
H_L(Y_t| X_{t-\Theta},\Theta) = \min_{\phi\in \Phi} \mathbb{E}_{Y,X,\Theta\sim P_{Y_t,X_{t-\Theta},\Theta}}[L(Y,\phi(X,\Theta))],
\end{align} 
where $\Phi$ is the set of all function mappings from $\mathcal X \times\mathcal D$ to $\mathcal A$. Because $\Lambda \subset \Phi, H_L(Y_t| X_{t-\Theta},\Theta) \leq \mathrm{err}_{\mathrm{training}}$. For {\blue notational convenience, we refer to $H_L(Y_t| X_{t-\Theta},\Theta)$ as an \emph{$L$-conditional entropy}}, because it is associated to a loss function $L$. By choosing different $L$, a broad class of $L$-conditional entropies is obtained.~In particular, Shannon's conditional entropy is derived if $L$ is the logarithmic loss function $L_{\log}(y,P_Y) = - \log P_Y(y)$. {\blue The optimal solution to \eqref{eq_TrainingErrorLB} is denoted as $\hat \phi_{P_{Y_t, X_{t-\Theta},\Theta}}$.}

{\blue Because} $\Phi$ contains all functions from $\mathcal{X}\times \mathcal D$ to $\mathcal{A}$, \eqref{eq_TrainingErrorLB} can be decomposed into a sequence of separated optimization problems, each optimizing an action $\phi(x, \theta)$ for given $(x, \theta) \in \mathcal X \times \mathcal D$ \cite{Dawid2004, farnia2016minimax}:
\begin{align} \label{L_condEntropy}
\!\!\!\!&H_L(Y_t| X_{t-\Theta},\Theta) \nonumber\\
\!\!\!\!=&\!\!\min_{\substack{\phi(x, \theta)\in \mathcal A
} } \!\!\sum_{\substack{x \in \mathcal X, \theta \in \mathcal D}} \!\! P_{X_{t-\Theta},\Theta}(x, \theta)\mathbb E_{Y\sim P_{Y_t|X_{t-\Theta}=x, \Theta=\theta}}[L(Y,\phi(x, \theta))] \nonumber\\
\!\!\!\!=&\!\!\!\sum_{\substack{x \in \mathcal X, \theta \in \mathcal D}} \!\!\!\! P_{X_{t-\Theta}, \Theta}(x, \theta) \!\!\min_{\phi(x, \theta)\in\mathcal A}\!\! E_{Y\sim P_{Y_t|X_{t-\Theta}=x, \Theta=\theta}}[L(Y,\phi(x, \theta))].\!\!\!\!
\end{align}
We note that problem \eqref{eq_trainingerror} cannot be decomposed in this way, because its function space $\Lambda$ is smaller than $\Phi$.  

If the action $a$ is {\blue selected without using any knowledge about $(X_{t-\Theta},\Theta)$, \eqref{eq_TrainingErrorLB} becomes \cite{Dawid2004, farnia2016minimax}}
\begin{align}\label{eq_Lentropy}
H_L(Y_t) = \min_{a\in\mathcal A} \mathbb{E}_{Y \sim P_{Y_t}}[L(Y,a)],
\end{align}
where $H_L(Y_t)$ is termed the $L$-\emph{entropy} of $Y_t$. {\violet We assume that the minimum on the right hand side of \eqref{eq_Lentropy} can be achieved by an action $a_{P_{Y_t}}$ in $\mathcal A$, which is called \emph{Bayes action} \cite{farnia2016minimax}.} If the Bayes actions are not unique, one can pick any such Bayes action as $a_{P_{Y_t}}$\cite{Dawid2014}.

{\blue If the distribution $P_{Y_t}$ in \eqref{eq_Lentropy} is changed as $P_{Y_t|X_{t-\Theta}=x, \Theta=\theta}$, we obtain the $L$-conditional entropy of $Y_t$ given $X_{t-\Theta}=x$ and $\Theta=\theta$:}
\begin{align}\label{given_L_condentropy}
\!\!\!&H_L(Y_t| X_{t-\Theta}=x,\Theta=\theta)\!\! \nonumber\\
=& \! \min_{a\in \mathcal A} \! \mathbb E_{Y\sim P_{Y_t|X_{t-\Theta}=x, \Theta=\theta}} [L(Y,a)] \nonumber\\
\!\!=& \!\!\!\!\!\! \min_{\phi(x, \theta)\in\mathcal A}\! \mathbb E_{Y\sim P_{Y_t|X_{t-\Theta}=x, \Theta=\theta}} [L(Y,\phi(x, \theta))].\!\!\!
\end{align}
{\violet Because the training label and the feature $(Y_t, X_t)$ are assumed to be independent of the training AoI $\Theta$, substituting \eqref{given_L_condentropy} into \eqref{L_condEntropy}, yields
\ifreport
(See Appendix \ref{pfreshness_aware_cond} for its proof)
\else
(See our technical report \cite{technical_report} for its proof)
\fi
\begin{align}\label{freshness_aware_cond}
\!\! H_L(Y_t| X_{t-\Theta},\Theta)\!=&\!\!\sum_{\substack{x \in \mathcal X, \theta \in \mathcal D}} \!\!\!\! P_{X_{t-\Theta}}(x) P_{\Theta}(\theta) H_L(Y_t| X_{t-\Theta}=x,\Theta=\theta)\!\!\! \nonumber\\
=&\sum_{\theta \in \mathcal D} \!\!\!\! P_{\Theta}(\theta)~H_L(Y_t| X_{t-\theta}).\!\!\! 
\end{align}}

{\blue We also need to define the \emph{$L$-cross entropy} between $\tilde Y_t$ and $Y_t$:} 
\begin{align} \label{cross-entropy}
H_L(\tilde Y_t; Y_t)= \mathbb{E}_{Y \sim P_{\tilde Y_t}}\left[L\left(Y, a_{P_{Y_t}}\right)\right].
\end{align}
{\blue Then, the $L$-\emph{divergence} $D_L(P_{\tilde Y_t} || P_{Y_t})$ of $P_{Y_t}$ from $P_{\tilde Y_t}$ can be expressed as \cite{Dawid2004, farnia2016minimax}
\begin{align}\label{divergence}
    D_L(P_{\tilde Y_t} || P_{Y_t})=&\mathbb E_{Y \sim P_{\tilde Y_t}}\left[L\left(Y, a_{P_{Y_t}}\right)\right]-\mathbb E_{Y \sim P_{\tilde Y_t}}\left[L\left(Y, a_{P_{\tilde Y_t}}\right)\right]\nonumber\\
    =&H_L(\tilde Y_t; Y_t)-H_L(\tilde Y_t)\geq 0.
\end{align}
The \emph{$L$-mutual information} $I_L(Y_t;X_t)$ is defined as \cite{Dawid2004, farnia2016minimax}
\begin{align}\label{MI}
I_L(Y_t; X_t)=& \mathbb E_{X \sim P_{X_t}}\left[D_L\left(P_{Y_t|X}||P_{Y_t}\right)\right]\nonumber\\
=&H_L(Y_t)-H_L(Y_t|X_t) \geq 0,
\end{align}
which measures the performance gain in predicting $Y_t$ by observing $X_t$. In general, $I_L(Y_t;X_t)$ $\neq$ $I_L(X_t;Y_t)$.} {\violet The $L$-conditional mutual information $I_L(Y_t; X_t | Z_t)$ is given by 
\begin{align}\label{CMI}
I_L(Y_t; X_t|Z_t)=& \mathbb E_{X, Z \sim P_{X_t, Z_t}}\left[D_L\left(P_{Y_t|X, Z}||P_{Y_t | Z}\right)\right]\nonumber\\
=&H_L(Y_t | Z_t)-H_L(Y_t|X_t, Z_t).
\end{align}}

\begin{figure*}[h]
  \centering
\begin{subfigure}{0.3\textwidth}
\includegraphics[width=\textwidth]{./Figure_Control/Control_loop.eps}
  \subcaption{Control System}
\end{subfigure}
% <— this is important. There should be no empty line here. 
\begin{subfigure}{0.3\textwidth}
\includegraphics[width=\textwidth]{./Figure_Control/DataTraces.eps}
  \subcaption{Time-series data}
\end{subfigure}
%
\begin{subfigure}{0.3\textwidth}
\includegraphics[width=\textwidth]{./Figure_Control/TrainingError.eps}
  \subcaption{Car Position and Velocity Prediction}
\end{subfigure}
%
\caption{(a) A Control System, where $A_p(t)$ and $S_p(t)$ are the action and state of the system at the plant and $A_c(t)$ and $S_c(t)$ are the action and state of the system at the controller (b) Time-series data of the action at the controller and state (car velocity and car position) at the plant, where there are $3$ action values $1, 0,$ and $-1$, respectively indicate (i) accelerate at the right, (ii) no acceleration, and (iii) accelerate at the left, and (c) Training error vs.~deterministic training AoI $\theta$ in predicting states at plant by using action at the controller.}
\label{fig:Training}
\end{figure*}


\ifreport
{\blue The relationship among $L$-divergence, Bregman divergence \cite{Dawid2004, Amari}, and $f$-divergence \cite{csiszar2004information} is discussed in Appendix \ref{InformationTheory2}. We note that any Bregman divergence is an $L$-divergence, and an $L$-divergence is a Bregman divergence only if $H_L(Y_t)$ is continuously differentiable and strictly concave in $\mathcal P_{Y_t}$ \cite{Dawid2004}. Examples of loss function $L$, $L$-entropy, and $L$-cross entropy are provided in Appendix \ref{InformationTheory1}.}
\else
{\blue he relationship among $L$-divergence, Bregman divergence \cite{Dawid2004, Amari}, and $f$-divergence \cite{csiszar2004information} is discussed in our technical report \cite{technical_report}. We note that any Bregman divergence is an $L$-divergence, and an $L$-divergence is a Bregman divergence only if $H_L(Y_t)$ is continuously differentiable and strictly concave in $\mathcal P_{Y_t}$ \cite{Dawid2004}. Examples of loss function $L$, $L$-entropy, and $L$-cross entropy are provided in \cite{technical_report}.}
\fi 

\subsection{Metrics for Inference Error}
{\blue If the trained predictor $\phi^*_{P_{Y_t, X_{t-\Theta},\Theta}}$ in \eqref{eq_inferenceerror} is replaced by the optimal solution $\hat \phi_{P_{Y_t, X_{t-\Theta},\Theta}}$ to \eqref{eq_TrainingErrorLB}, then $\mathrm{err}_{\mathrm{inference}}$ becomes an \emph{$L$-conditional cross entropy} $H_L(Y_{t}; $ $\tilde Y_{t} | \tilde X_{t-\Delta}, \Delta)$, which is given by}
\begin{align}\label{L-CondCrossEntropy}
&H_L(\tilde Y_{t}; Y_{t} | \tilde X_{t-\Delta}, \Delta) \nonumber\\
=&\mathbb{E}_{Y,X,\Delta\sim P_{\tilde Y_t,\tilde X_{t- \Delta},\Delta}}\left[L\left(Y,\hat \phi_{P_{Y_t, X_{t-\Theta},\Theta}}(X,\Delta)\right)\right].
\end{align} 
{\blue If the function space $\Lambda$ is sufficiently large, the difference between $\mathrm{err}_{\mathrm{inference}}$ and $H_L(\tilde Y_{t}; Y_{t} | \tilde X_{t-\Delta}, \Delta)$ is small.} 
Since $\{(Y_t, X_t), t \in \mathbb Z\}$ is independent of $\Theta$ and $\{(\tilde Y_t, \tilde X_t), t \in \mathbb Z\}$ is independent of $\Delta$, the $L$-conditional cross entropy in \eqref{L-CondCrossEntropy} can be decomposed as 
\ifreport
(See Appendix \ref{pDecomposed_Cross_entropy} for its proof)
\else
(See our technical report \cite{technical_report} for its proof)
\fi
\begin{align}\label{Decomposed_Cross_entropy}
H_L(\tilde Y_t;Y_t| \tilde X_{t-\Delta}, \Delta) = \sum_{\delta \in \mathcal D} P_\Delta(\delta)~H_L(\tilde Y_t;Y_t| \tilde X_{t-\delta}).
\end{align}
{\violet Similar to \eqref{divergence}, we can get
\begin{align}\label{L-ConCrossEntropy1}
\!\!\!\!\!H_L(\tilde Y_{t}; Y_{t} | \tilde X_{t-\Delta}, \Delta) =&H_L(\tilde Y_{t} | \tilde X_{t-\Delta}, \Delta)+\sum_{x \in \mathcal X, \delta \in \mathcal D} P_{\tilde X_{t- \Delta},\Delta}(x, \delta)\nonumber\\
&\!\!\times D_L\left(P_{\tilde Y_t | \tilde X_{t-\Delta}=x, \Delta=\delta} || P_{Y_t | X_{t-\Theta}=x, \Theta=\delta}\right).\!\!\!
\end{align}
Because the $L$-divergence in \eqref{L-ConCrossEntropy1} is non-negative, we have}
\begin{align}\label{lowerbound_inference}
H_L(\tilde Y_{t}; Y_{t} | \tilde X_{t-\Delta}, \Delta) \geq H_L(\tilde Y_{t} | \tilde X_{t-\Delta}, \Delta).
\end{align}


%This case is of particular interest for two reasons: (i) it provides a fundamental risk lower bound for any ERM-based supervised learning algorithm;  and (ii) it is convenient in our information-theoretic analysis because \eqref{cond_entropy1} can be decomposed into a series of separable optimization problems, as we will see soon in \eqref{cond_Entropy}. For this choice of $\Psi$, the minimum risk $H_L(Y|X)$ in \eqref{cond_entropy1} is called the \emph{generalized conditional entropy} of $Y$ given $X$ \cite{David_Tse}. 



==> SystemModel.tex <==
\section{System Model}
